BoBDeLaN: Bounded-Bandwidth Context Adaptation for Deep Lagrangian Robot Control

Learned physics-based models provide structure for robot control, but uncertain payloads and unmodeled dynamics limit their predictive accuracy. Context-aware Deep Lagrangian Networks enable adaptation through a latent context inferred from measurement histories while retaining Lagrangian structure for each fixed context. However, this structure alone does not constrain sensitivity to measurement disturbances. We introduce BoBDeLaN, which combines a contracting, gain-bounded Recurrent Equilibrium Network context encoder with stable linear filtering to shape disturbance sensitivity across frequencies. This architecture guarantees exponential forgetting of the recurrent initialization and admits a finite-horizon, frequency-weighted bound on context perturbations, which extends to residual torque prediction under a Lipschitz continuity assumption on the context-conditioned dynamics model. We evaluate a low-pass realization within model predictive control on simulated and real hardware manipulation tasks, together with frequency-sensitivity analysis on real-robot data. Compared with an LSTM encoder using the same input filter, BoBDeLaN exhibits reduced high-frequency context sensitivity, lower residual torque prediction error, and smoother motion, with less degradation under injected disturbances.

==> Results/sim_id_v1.tex <==
\begin{table}[t]
\centering
\caption{Average joint tracking RMSE of the MPC for the four models over the 600 simulated trajectories (in-distribution payloads).}
\label{tab:tracking_id}
\begin{tabular}{lccccccc}
\hline
Model & $j_1$ & $j_2$ & $j_3$ & $j_4$ & $j_5$ & $j_6$ & $j_7$ \\
\hline
\multicolumn{8}{c}{Position tracking error $\bar{e}_\mathrm{q}$ [rad]} \\
Nominal & 0.019 & 0.051 & 0.037 & 0.082 & 0.117 & 0.131 & 0.117 \\
DeLaN-LSTM & 0.015 & \textbf{0.026} & 0.024 & 0.047 & 0.040 & 0.060 & 0.036 \\
DeLaN-LSTM-j1 & 0.018 & 0.031 & 0.024 & \textbf{0.041} & 0.038 & \textbf{0.042} & 0.035 \\
DeLaN-REN & \textbf{0.009} & 0.067 & \textbf{0.019} & 0.054 & \textbf{0.029} & 0.062 & \textbf{0.022} \\
\hline
\multicolumn{8}{c}{Velocity tracking error $\bar{e}_{\dot{\mathrm{q}}}$ [rad/s]} \\
Nominal & 0.044 & \textbf{0.062} & 0.069 & \textbf{0.066} & 0.169 & \textbf{0.170} & 0.184 \\
DeLaN-LSTM & 0.166 & 0.138 & 0.187 & 0.171 & 0.368 & 0.342 & 0.374 \\
DeLaN-LSTM-j1 & 0.131 & 0.130 & 0.143 & 0.144 & 0.326 & 0.273 & 0.401 \\
DeLaN-REN & \textbf{0.032} & 0.101 & \textbf{0.049} & 0.112 & \textbf{0.074} & 0.171 & \textbf{0.084} \\
\hline
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Average residual torque RMSE and one-step joint velocity prediction RMSE for the four models over the 600 simulated trajectories (in-distribution payloads).}
\label{tab:prediction_id}
\begin{tabular}{lccccccc}
\hline
Model & $j_1$ & $j_2$ & $j_3$ & $j_4$ & $j_5$ & $j_6$ & $j_7$ \\
\hline
\multicolumn{8}{c}{Residual torque error $\bar{e}_\mathrm{r}$ [Nm]} \\
Nominal & 1.06 & 6.07 & 2.78 & 6.58 & 2.02 & 2.52 & 1.72 \\
DeLaN-LSTM & 7.36 & 3.48 & 5.19 & 3.68 & 2.31 & 2.05 & 2.50 \\
DeLaN-LSTM-j1 & 3.48 & 3.21 & 4.51 & 3.17 & 2.16 & 1.95 & 2.26 \\
DeLaN-REN & \textbf{0.62} & \textbf{0.93} & \textbf{0.86} & \textbf{2.23} & \textbf{0.85} & \textbf{1.06} & \textbf{0.87} \\
\hline
\multicolumn{8}{c}{Velocity prediction error $\bar{e}_{\dot{\mathrm{q}}}$ [rad/s]} \\
Nominal & 0.0690 & 0.0683 & 0.0932 & 0.1015 & 0.3290 & 0.3459 & 0.3616 \\
DeLaN-LSTM & 0.1412 & 0.0526 & 0.1344 & 0.0752 & 0.2097 & 0.1869 & 0.2459 \\
DeLaN-LSTM-j1 & 0.0937 & 0.0481 & 0.0993 & 0.0549 & 0.1744 & 0.1524 & 0.2310 \\
DeLaN-REN & \textbf{0.0193} & \textbf{0.0173} & \textbf{0.0206} & \textbf{0.0492} & \textbf{0.0312} & \textbf{0.0953} & \textbf{0.0528} \\
\hline
\end{tabular}
\end{table}

